Feature selection in machine learning: R\'enyi min-entropy vs Shannon entropy

Feature selection, in the context of machine learning, is the process of separating the highly predictive feature from those that might be irrelevant or redundant. Information theory has been recognized as a useful concept for this task, as the prediction power stems from the correlation, i.e., the mutual information, between features and labels. Many algorithms for feature selection in the literature have adopted the Shannon-entropy-based mutual information. In this paper, we explore the possibility of using R\'enyi min-entropy instead. In particular, we propose an algorithm based on a notion of conditional R\'enyi min-entropy that has been recently adopted in the field of security and privacy, and which is strictly related to the Bayes error. We prove that in general the two approaches are incomparable, in the sense that we show that we can construct datasets on which the R\'enyi-based algorithm performs better than the corresponding Shannon-based one, and datasets on which the situation is reversed. In practice, however, when considering datasets of real data, it seems that the R\'enyi-based algorithm tends to outperform the other one. We have effectuate several experiments on the BASEHOCK, SEMEION, and GISETTE datasets, and in all of them we have indeed observed that the R\'enyi-based algorithm gives better results.

==> main-save.bbl.tex <==
 \begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{Alvim:12:CSF}
Alvim, M.S., Chatzikokolakis, K., Palamidessi, C., Smith, G.: Measuring
  information leakage using generalized gain functions. In: Proc. of CSF. pp.
  265--279 (2012)

\bibitem{Amaldi:98:TCS}
Amaldi, E., Kann, V.: On the approximability of minimizing nonzero variables or
  unsatisfied relations in linear systems. Theor. Comput. Sci
  \textbf{209}(1-2),  237--260 (1998)

\bibitem{Arimoto:75:CMJB}
Arimoto, S.: Information measures and capacity of order $\alpha$ for discrete
  memoryless channels. In: Topics in Information Theory, Proc. Coll. Math. Soc.
  Janos Bolyai. pp. 41--52 (1975)

\bibitem{Battiti:94:TNN}
Battiti, R.: Using mutual information for selecting features in supervised
  neural net learning. IEEE Trans. Neural Networks  \textbf{5}(4),  537--550
  (1994)

\bibitem{Bennesar:15:ESA}
\revision{Bennasar, M., Hicks, Y., Setchi, R.: Feature selection using joint mutual
  information maximisation. Expert Syst. Appl  \textbf{42}(22),  8520--8532
  (2015)}

\bibitem{Brown:12:JMLR}
\revision{Brown, G., Pocock, A.C., Zhao, M.J., Luj{\'a}n, M.: Conditional likelihood
  maximisation: A unifying framework for information theoretic feature
  selection. MLR  \textbf{13},  27--66 (2012)}
%  ,
%  \url{http://dl.acm.org/citation.cfm?id=2188387}

\bibitem{Cachin:97:PhDThesis}
Cachin, C.: Entropy Measures and Unconditional Security in Cryptography. Ph.D.
  thesis, {ETH} Zurich (1997)
%  , reprint as vol.~1 of {\em ETH Series in
%  Information Security and Cryptography}, {ISBN} 3-89649-185-7,
%  {H}artung-{G}orre {V}erlag, {K}onstanz, 1997

\bibitem{Cai:18:Neurocomputing}
\revision{Cai, J., Luo, J., Wang, S., Yang, S.: Feature selection in machine learning: A
  new perspective. Neurocomputing  \textbf{300},  70 -- 79 (2018)}

\bibitem{Chang:11:ACM}
Chang, C.C., Lin, C.J.: {LIBSVM}: A library for support vector machines. ACM
  Transactions on Intelligent Systems and Technology  \textbf{2},  27:1--27:27
  (2011)
%  , software available at \url{http://www.csie.ntu.edu.tw/~cjlin/libsvm}

\bibitem{Cover:91:BOOK}
Cover, T.M., Thomas, J.A.: Elements of Information Theory. J. Wiley \& Sons,
  Inc. (1991)

\bibitem{Csiszar:95:TIT}
Csisz{\'a}r, I.: {Generalized cutoff rates and R{\'e}nyi's information
  measures}. Trans. on Information Theory  \textbf{41}(1),  26--34 (1995)

\bibitem{Endo:13:CIARP}
Endo, T., Kudo, M.: Weighted na{\"\i}ve Bayes classifiers by R\'enyi entropy. In:
Proc. of CIARP 2013. LNCS, vol.~8258, pp. 149--156. Springer (2013)

\bibitem{Fleuret:04:JMLR}
Fleuret, F.: Fast binary feature selection with conditional mutual information.
  JMLR \textbf{5},  1531--1555 
(2004),
%  \url{http://www.jmlr.org/papers/volume5/fleuret04a/fleuret04a.pdf}

\bibitem{Guyon:03:MLR}
Guyon, I., Elisseeff, A.: An introduction to variable and feature selection.
  JMLR  \textbf{3}
%  ,  1157--1182 
  (2003)

\bibitem{Jain:00:TPAMI}
Jain, A.K., Duin, R.P.W., Mao, J.: Statistical pattern recognition: A review.
  IEEE Trans. on Pattern Analysis and Machine Intelligence  \textbf{22}(1),
  4--37 (2000)

\bibitem{Kohavi:97:AI}
Kohavi, R., John, G.: Wrappers for feature subset selection. Art. Int.
   \textbf{97},  273--324 (1997)

\bibitem{Liu:05:TKDE}
Liu, H., Yu, L.: Toward integrating feature selection algorithms for
  classification and clustering. IEEE Trans. on Knowledge and Data Engineering
  \textbf{17}(4),  491--502 (2005)

\bibitem{Liu:18:KBS}
\revision{Liu, J., Lin, Y., Wu, S., Wang, C.: Online multi-label group feature selection.
  Knowledge-Based Systems  \textbf{143},  42 -- 57 (2018)}

\bibitem{Nakariyakul:18:KBS}
\revision{Nakariyakul, S.: High-dimensional hybrid feature selection using interaction
  information-guided search. Knowledge-Based Systems  \textbf{145},  59 -- 66
  (2018)}

\bibitem{Palamidessi:18:REPORT}
Palamidessi, C., Romanelli, M.: Feature selection with r\'enyi min-entropy.
  Tech. rep., INRIA (2018),  available at
  \url{https://hal.archives-ouvertes.fr/hal-01830177}

\bibitem{Pedregosa:11:JML}
Pedregosa, F. et al.: Machine learning in {P}ython. JMLR  \textbf{12},  2825--2830 (2011)

\bibitem{Peng:05:TPAMI}
Peng, H., Long, F., Ding, C.H.Q.: Feature selection based on mutual
  information: Criteria of max-dependency, max-relevance, and min-redundancy.
%  IEEE Trans. Pattern Anal. Mach. Intell 
  TPAMI \textbf{27}(8),  1226--1238 (2005),
%  \url{http://doi.ieeecomputersociety.org/10.1109/TPAMI.2005.159}

\bibitem{Renyi:61:Berkeley}
R\'enyi, A.: {On Measures of Entropy and Information}. In: Proceedings of the
  4th Berkeley Symposium on Mathematics, Statistics, and Probability. pp.
  547--561 (1961)

\bibitem{Sheikhpour:17:PR}
\revision{Sheikhpour, R., Sarram, M.A., Gharaghani, S., Chahooki, M.A.Z.: A survey on
  semi-supervised feature selection methods. Pattern Recognition  \textbf{64},
  141 -- 158 (2017)}

\bibitem{Sibson:69:ZWG}
Sibson, R.: Information radius. Z. Wahrscheinlichkeitsth. und Verw. Geb
  \textbf{14},  149--161 (1969)

\bibitem{Smith:09:FOSSACS}
Smith, G.: On the foundations of quantitative information flow. In: Proc. of
  FOSSACS. LNCS, vol.~5504, pp. 288--302. Springer (2009)

\bibitem{Snoek:12:Corr}
Snoek, J., Larochelle, H., Adams, R.P.: Practical \revision{ {B}ayesian } optimization of
  machine learning algorithms. CoRR  \textbf{abs/1206.2944} (2012),
  \url{http://arxiv.org/abs/1206.2944}

\bibitem{Vergara:14:NCA}
\revision{Vergara, J.R., Est{\'e}vez, P.A.: A review of feature selection methods based
  on mutual information. Neural Computing and Applications  \textbf{24}(1),
  175--186 (2014)}

\bibitem{Yang:99:AIDA}
Yang, H.H., Moody, J.: Feature selection based on joint mutual information. In:
 Proc. of International ICSC Symposium on Advances in Intelligent
  Data Analysis. pp. 22--25 (1999)

\end{thebibliography}


